A category for bijective combinatorics

The category of matchings between finite sets extends to the category of cobordisms of signed sets. A chain of cobordisms that starts and ends with unsigned sets A and B yields a matching from A to B. This is a convenient way to package the involution principle of Garsia and Milne, which reveals itself to have little to do with involutions.

==> zzz_dot_bib <==
@article {fp,
    AUTHOR = {Feldman, David and Propp, James},
     TITLE = {Producing new bijections from old},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {113},
      YEAR = {1995},
     PAGES = {1--44}
}

@article {schwartz:fourA,
    AUTHOR = {Schwartz, Rich Evan},
     TITLE = {Pan [G]alactic [D]ivision},
   JOURNAL = {Math. Intelligencer},
  FJOURNAL = {The Mathematical Intelligencer},
    VOLUME = {37},
      YEAR = {2015},
    NUMBER = {3},
     PAGES = {8--10},
eprint={arXiv:1504.02179 [math.CO]},
note={\url{http://arxiv.org/abs/1504.02179}},
}

}

@book{hinkis,
author="Arie Hinkis",
title="Proofs of the Cantor-Bernstein Theorem: A Mathematical Excursion",
year="2013",
publisher="Birkhauser"
}



@misc{conwaydoyle:three,
title={Division by three},
author = {Peter G. Doyle and John Horton Conway},
year="1994",
eprint={arXiv:math/0605779 [math.LO]},
note={\url{http://arxiv.org/abs/math/0605779}},
}

@misc{doyleqiu:four,
title={Division by four},
author = {Peter G. Doyle and Cecil Qiu},
year="2015",
eprint={arXiv:1504.01402 [math.LO]},
note={\url{http://arxiv.org/abs/1504.01402}},
}

@misc{bajpaidoyle:equivariant,
title={Equivariant division},
author = {Prajeet Bajpai and Peter G. Doyle},
year="2016",
eprint={arXiv:1704.04089 [math.CO]},
note={\url{http://arxiv.org/abs/1704.04089}},
}

@book{bachmann:transfinite,
	author =	"H. Bachmann",
	title =		"Transfinite Zahlen (Zweite Auflage)",
	publisher =	"Springer",
	address =	"Berlin",
	year =		"1967"
}
@article{bernstein:mengenlehre,
	author =	"F. Bernstein",
	title =		"Untersuchungen aus der {M}engenlehre",
	journal =	"Math. Ann.",
	volume =	"61",
	year =		"1905",
	pages =		"117-154"
}
@article{garsiaMilne:rogers,
	author =	"A. M. Garsia and S. C. Milne",
	title =		"A {R}ogers-{R}amanujan bijection",
	journal =	"J. Combin. Theory, Series A",
	volume =	"31",
	year =		"1981",
	pages =		"289-339"
}
@article{garsiaMilne:method,
	author =	"A. M. Garsia and S. C. Milne",
	title =		"Method for constructing bijections for classical partition identities",
	journal =	"Proc. Natl. Acad. Sci. USA",
	volume =	"78",
	year =		"1981",
	pages =		"2026-2028"
}

@book{jech:setTheory,
	author =	"T. Jech",
	title =		"Set Theory",
	publisher =	"Academic Press",
	address =	"New York",
	year =		"1978"
}

@article{lindenbaumTarski:ensembles,
	author =	"A. Lindenbaum and A. Tarski",
	title =		"Communication sur les recherches de la th\'{e}orie des ensembles",
	journal =	"Comptes Rendus des s\'{e}ances de la Soci\'{e}t\'{e} des Sciences et des Letters de Varsovie, Classe {I}{I}{I}",
	volume =	"19",
	year =		"1926",
	pages =		"299-330"
}

@book{nelson:predicative,
	author =	"E. Nelson",
	title =		"Predicative Arithmetic",
	publisher =	"Princeton University Press",
	address =	"Princeton",
	year =		"1986"
}

@article{remmel:partition,
	author =	"J. B. Remmel",
	title =		"Bijective proofs of some classical partition identities",
	journal =	"J. Combin. Theory, Series A",
	volume =	"33",
	year =		"1982",
	pages =		"273-286"
}

@article{sierpinski:two,
	author =	"W. Sierpinski",
	title =		"Sur l'\'{e}galit\'{e} $2m=2n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"3",
	year =		"1922",
	pages =		"1-6"
}

@article{sierpinski:leq,
	author =	"W. Sierpinski",
	title =		"Sur l'implication $2m\leq 2n \rightarrow m \leq n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"34",
	year =		"1947",
	pages =		"148-154"
}

@article{tarski:cancellation,
	author =	"A. Tarski",
	title =		"Cancellation laws in the arithmetic of cardinals",
	journal =	"Fundamenta Mathematica",
	volume =	"36",
	year =		"1949",
	pages =		"77-92"
}

@article{schwartz:four,
title={{P}an {G}alactic {D}ivision},
author = {Rich Schwartz},
journal={Math. Intell.},
volume={37},
number={3},
pages={8-10},
year={2015},
eprint={arXiv:1504.02179 [math.CO]},
note={\url{http://arxiv.org/abs/1504.02179}},
}

@book{hall:groups,
title={The Theory of Groups},
author={Marshall Hall},
year={1959}
}

@book {jech:choice,
    AUTHOR = {Jech, Thomas J.},
     TITLE = {The axiom of choice},
      YEAR = {1973}
}

@article{koenig,
author={Koenig, Jules},
title={Sur le th\'{e}orie des ensembles},
journal={C. R. H\'eb. Acad. Sci. Paris},
year={1906},
volume={143},
pages={110-112},
note={Reprinted here as Appendix \ref{app}}
}

@phdthesis{picciotto:thesis,
  author       = {Sally Picciotto}, 
  title        = {How to encode a tree},
  school       = {UCSD},
  year         = 1999,
eprint={arXiv:1710.08463 [math.CO]},
note={\url{http://arxiv.org/abs/1710.08463}}
}

@book{stantonwhite,
    AUTHOR = {Stanton, Dennis and White, Dennis},
     TITLE = {Constructive Combinatorics},
 PUBLISHER = {Springer},
      YEAR = {1986}
}

